RoLoRA: Fine-tuning Rotated Outlier-free LLMs for Effective Weight-Activation Quantization

Low-Rank Adaptation (LoRA), as a representative Parameter-Efficient Fine-Tuning (PEFT)method, significantly enhances the training efficiency by updating only a small portion of the weights in Large Language Models (LLMs). Recently, weight-only quantization techniques have also been applied to LoRA methods to reduce the memory footprint of fine-tuning. However, applying weight-activation quantization to the LoRA pipeline is under-explored, and we observe substantial performance degradation primarily due to the presence of activation outliers. In this work, we propose RoLoRA, the first LoRA-based scheme for effective weight-activation quantization. RoLoRA utilizes rotation for outlier elimination and proposes rotation-aware fine-tuning to preserve the outlier-free characteristics in rotated LLMs. Experimental results show RoLoRA consistently improves low-bit LoRA convergence and post-training quantization robustness in weight-activation settings. We evaluate RoLoRA across LLaMA2-7B/13B, LLaMA3-8B models, achieving up to 29.5% absolute accuracy gain of 4-bit weight-activation quantized LLaMA2- 13B on commonsense reasoning tasks compared to LoRA baseline. We further demonstrate its effectiveness on Large Multimodal Models (LLaVA-1.5-7B). Codes are available at https://github.com/HuangOwen/RoLoRA

==> tables/llama_main.tex <==
\begin{table*}[t]
\renewcommand\arraystretch{1} 
\centering
\caption{Comparison of the averaged accuracy on seven Zero-shot Common Sense Reasoning (ZCSR) tasks and MMLU benchmark across LLaMA series. The detailed accuracy for each tasks are listed in Table~\ref{tab:zeroshot_full} and Table~\ref{tab:mmlu_full}.}  \vspace{-1ex}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{c|c|c|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{\#Bits}} & \multirow{2}{*}{\textbf{Quantizer}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{LLaMA-2 7B}} & \multicolumn{2}{c|}{\textbf{LLaMA-2 13B}} & \multicolumn{2}{c}{\textbf{LLaMA-3 8B}} \\ 
\cmidrule{4-9}
 &  &  & ZCSR$^7$ Avg. & MMLU$^4$ Avg. & ZCSR$^7$ Avg. & MMLU$^4$ Avg. & ZCSR$^7$ Avg. & MMLU$^4$ Avg. \\
\midrule
FP16  & - & LoRA & 68.4 & 43.5 & 70.5 & 52.4 & 70.0 & 62.7 \\
\midrule
\multirow{4}{*}{W4A4}  & \multirow{2}{*}{RTN} & LoRA & 35.8 & 23.5 & 34.4 & 24.2 & 36.7 & 23.3 \\
&  & \rowcolor{gray!10}{\methodname} & \bf 54.1 (\textcolor{mygreen}{$\uparrow$18.3}) & \bf 25.8 (\textcolor{mygreen}{$\uparrow$2.3})& \bf 58.7 (\textcolor{mygreen}{$\uparrow$24.3})& \bf 30.5 (\textcolor{mygreen}{$\uparrow$6.3})& \bf 50.0 (\textcolor{mygreen}{$\uparrow$13.3})& \bf 32.1 (\textcolor{mygreen}{$\uparrow$8.8})\\
\cmidrule{2-9}
& \multirow{2}{*}{GPTQ} & LoRA & 37.0  & 23.5 & 34.4 & 24.4 & 36.6 & 23.9 \\
&  & \rowcolor{gray!10}{\methodname} & \bf 62.3 (\textcolor{mygreen}{$\uparrow$25.3})& \bf 31.0 (\textcolor{mygreen}{$\uparrow$7.5})& \bf 63.9 (\textcolor{mygreen}{$\uparrow$29.5})& \bf 38.9 (\textcolor{mygreen}{$\uparrow$14.5})& \bf 56.6 (\textcolor{mygreen}{$\uparrow$20.0})& \bf 38.5 (\textcolor{mygreen}{$\uparrow$14.6})\\
\midrule
\multirow{4}{*}{W6A6}  & \multirow{2}{*}{RTN} & LoRA & 65.3 & 35.9 & 67.3 & 47.3 & 67.7 & 55.3 \\
&  & \rowcolor{gray!10}{\methodname} & \bf 66.8 (\textcolor{mygreen}{$\uparrow$1.5})& \bf 40.5 (\textcolor{mygreen}{$\uparrow$4.6})& \bf 68.4 (\textcolor{mygreen}{$\uparrow$1.1})& \bf 47.7 (\textcolor{mygreen}{$\uparrow$0.4})& \bf 67.8 (\textcolor{mygreen}{$\uparrow$0.1})& \bf 59.4 (\textcolor{mygreen}{$\uparrow$4.1})\\
\cmidrule{2-9}
& \multirow{2}{*}{GPTQ} & LoRA & 65.5 & 35.7 & 68.0 & 47.6 & 67.8 & 54.3 \\
&  & \rowcolor{gray!10}{\methodname} & \bf 67.1 (\textcolor{mygreen}{$\uparrow$1.6})& \bf 40.8 (\textcolor{mygreen}{$\uparrow$5.1})& \bf 68.8 (\textcolor{mygreen}{$\uparrow$0.8})& \bf 47.9 (\textcolor{mygreen}{$\uparrow$0.3})& \bf 68.1 (\textcolor{mygreen}{$\uparrow$0.3})& \bf 59.4 (\textcolor{mygreen}{$\uparrow$5.1})\\
\bottomrule 
\end{tabular}}
\label{tab:main_llama}
\end{table*} 

==> tables/llama_qlora.tex <==
\begin{table*}[btp]
\centering
\caption{Comparison of the averaged accuracy of different Low-bit LoRA methods on Zero-shot Common Sense Reasoning tasks and MMLU benchmark on LLaMA2-7B.} \label{tab:qlora}
\vspace{-1ex}
\setlength{\tabcolsep}{1mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|c|ccccccc:c|cccc:c}
\toprule
\textbf{\#Bits} & \textbf{Quantizer} & \textbf{Method} & \textbf{BoolQ} & \textbf{PIQA} & \textbf{HellaS.} & \textbf{WinoG.}  & \textbf{Arc-e} & \textbf{Arc-c} & \textbf{OBQA} & \textbf{Avg.}  & \textbf{Hums.} & \textbf{STEM} & \textbf{Social} & \textbf{Other} & \textbf{Avg.} \\ 
\midrule
& \multirow{4}{*}{RTN} & QLoRA~\cite{dettmers2024qlora} & 47.1 &51.5 &27.5 &49.1 &28.4 &24.6 &25.4 &36.2 &24.1 &24.7 &22.9 &21.8 &23.5 \\
&  & LoftQ~\cite{li2024loftq} & 51.5 &50.8 &26.6 &50.4 &27.5 &26.0 &25.0 & \underline{36.8} &23.9 &24.0 &22.2 &22.2 &23.2  \\
\multirow{2}{*}{W4A16}&  & IR-QLoRA~\cite{qin2024accurate} & 45.5 &49.7 &26.7 &50.6 &25.7 &26.8 &26.8 &36.0 &24.3 &24.6 &23.9 &21.9 &\underline{23.7} \\
\multirow{2}{*}{$\downarrow$}&  & \rowcolor{gray!10}{\methodname} & 59.9 &60.5 &43.5 &51.8 &43.7 &28.6 &28.8 &\bf 45.3 (\textcolor{mygreen}{$\uparrow$8.5})&24.7 &25.3 &23.6 &24.3 &\bf 24.5 (\textcolor{mygreen}{$\uparrow$0.8})\\
\cmidrule{2-16}
\multirow{2}{*}{W4A4}& \multirow{4}{*}{GPTQ} & QLoRA~\cite{dettmers2024qlora} & 51.4 &51.6 &27.7 &51.9 &29.6 &25.3 &26.4 & \underline{37.7} &24.9 &24.0 &22.2 &22.5 &23.6  \\
&  & LoftQ~\cite{li2024loftq} & 55.9 &49.2 &27.2 &49.1 &26.6 &26.1 &24 &36.9 &24.1 &23.8 &23.3 &22.7 &23.6  \\
&  & IR-QLoRA~\cite{qin2024accurate} & 51.1 &49.8 &27.6 &49.3 &27.6 &24.6 &27.4 &36.8 &24.6 &24.8 &22.9 &22.7 & \underline{23.9} \\
&  & \rowcolor{gray!10}{\methodname} & 68.7 &73.1 &66.8 &61.3 &61.2 &37.8 &38.2 &\bf 58.2 (\textcolor{mygreen}{$\uparrow$20.5}) &28.3 &32.7 &32.3 &27.2 &\bf 29.9 (\textcolor{mygreen}{$\uparrow$6.0})\\
\noalign{\vspace{0.2em}}
\bottomrule
\end{tabular}}   \vspace{-1ex}
\end{table*}    

==> tables/llava_bench.tex <==
\begin{table}[h] 
\caption{Comparison of the W4A4 quantization performance on LLaVA-Bench of LLaVA-1.5-7B.}\label{tab:llava_bench}
\vspace{-1ex}
\centering
\resizebox{0.48\textwidth}{!}{\begin{tabular}{c|c|ccccc}
\toprule
\textbf{\#Bits} & \textbf{Quantizer} & \textbf{Method} & \textbf{Conv.} & \textbf{Detail} & \textbf{Reas.} & \textbf{Overall}  \\ 
\midrule
\multirow{4}{*}{W4A4}  & \multirow{2}{*}{RTN} & LoRA &  43.2 & 29.6 & 31.6 & 34.9 \\
&  & \rowcolor{gray!10}{\methodname} & 68.8 & 40.5 & 51.9 & \bf 53.8 (\textcolor{mygreen}{$\uparrow$18.9})\\
\cmidrule{2-7}
& \multirow{2}{*}{GPTQ} & LoRA & 70.6 & 41.8 & 47.9 & 53.5 \\
&  & \rowcolor{gray!10}{\methodname} & 67.5 & 48.3 & 66.2 & \bf 60.8 (\textcolor{mygreen}{$\uparrow$7.3}) \\
\bottomrule
\end{tabular}}  
\end{table}

==> tables/llava_example.tex <==
\begin{table}[t]
\centering
\begin{minipage}{1.0\columnwidth}\vspace{0mm}    
\centering
\begin{tcolorbox} 
    \centering
      \footnotesize
    \begin{tabular}{p{0.95\columnwidth}c}
\centering\includegraphics[height=4cm]{latex/figures/coco_2014val_000000385873.jpg} &\\
 {\bf Question:} User: Explain the visual content of the image \textcolor{blue}{in great detail}. (category: ``detail'') &\\
 \hrulefill & \\

{\bf GPT-4 Response:} The image displays three open pizza boxes with pizzas inside. The first pizza box, situated to the left, contains a smaller pizza. The second pizza box, positioned in the middle, features a larger pizza topped with tortilla chips. The third pizza box, located to the right, contains another smaller pizza. Beside the large pizza, there are two side orders of sauce in bowls, accompanying the delicious meal. The arrangement showcases a delicious spread of pizzas, inviting everyone to enjoy their different flavors and sizes.& \\
\hrulefill & \\

{\bf LoRA$\xrightarrow{\text{GPTQ}}$W4A4:} The image shows a pizza.&\\
\hrulefill & \\
{\bf \methodname$\xrightarrow{\text{GPTQ}}$W4A4:} The image features a pizza with \textcolor{blue}{a variety of toppings, including cheese, pepperonies, and chicken}. There are three pizzas in total, with one of them being a pizza with chicken. The pizzas are placed in a \textcolor{blue}{cardboard box}, which is open and ready for the pizzas. The pizzas are served in a box, making it a convenient and portable meal option.&\\
    \end{tabular}
\end{tcolorbox}
\vspace{-2ex}
\caption{LLaVA-1.5-7B W4A4 quantization evaluation on the example from LLaVA-Bench.}
    \label{tab:llava_example}
\end{minipage} \vspace{-3ex}
\end{table} 
